TiK-means: $K$-means clustering for skewed groups

The $K$-means algorithm is extended to allow for partitioning of skewed groups. Our algorithm is called TiK-Means and contributes a $K$-means type algorithm that assigns observations to groups while estimating their skewness-transformation parameters. The resulting groups and transformation reveal general-structured clusters that can be explained by inverting the estimated transformation. Further, a modification of the jump statistic chooses the number of groups. Our algorithm is evaluated on simulated and real-life datasets and then applied to a long-standing astronomical dispute regarding the distinct kinds of gamma ray bursts.

==> a00-preamble.tex <==
%\usepackage{dsfont}
\usepackage{booktabs}
\usepackage{tabularx}
\usepackage{subfloat}
\usepackage{colortbl}
\usepackage{graphicx}
\usepackage{verbatim}
\usepackage{amssymb}
\usepackage{amsmath}
\usepackage{multirow}
\usepackage{url}
\usepackage{rotating}
\usepackage{wrapfig}
\usepackage{helvet}
\usepackage{pdflscape}
\usepackage{placeins}
\usepackage{afterpage}
\usepackage{xcolor}


\usepackage{cleveref}
\usepackage{animate} 
\usepackage{multimedia}

%\usepackage[margin=1in]{geometry} % to get margins of 0.9 on all
                                % four sides
\usepackage{mdwlist} %http://www.terminally-incoherent.com/blog/2007/09/19/latex-squeezing-the-vertical-white-space/
%\usepackage[affil-it]{authblk} 
\RequirePackage{setspace}
\RequirePackage{caption}

%\captionsetup[table]{font={stretch=1.4}}     %% change 1.2 as you like
%\captionsetup[figure]{font={stretch=1.4}}    %% change 1.2 as you like
%\captionsetup{font={stretch=1.2}} 
%BLINDING
\captionsetup{font={it,stretch=1.2}}
%\captionsetup{font={it,stretch=1}}
% https://tex.stackexchange.com/questions/153334/change-the-baselinestretch-line-spacing-only-for-figure-captions/170533#170533
%\usepackage[compact]{titlesec}
%\titlespacing{\section}{0pt}{*1}{*1}
%\titlespacing{\subsection}{0pt}{*1}{*1}
%\titlespacing{\subsubsection}{0pt}{*1}{*1}
%\titlespacing{\paragraph}{0pt}{*1}{*1}
%\titlespacing{\subparagraph}{0pt}{*1}{*1}

%% make colors for table coloring
\definecolor{ggplot1}{HTML}{4f9b7a}
\definecolor{ggplot2}{HTML}{b0cfe1}
\definecolor{ggplot3}{HTML}{d44f8f}
\definecolor{ggplot4}{HTML}{deac42}
\definecolor{ggplot5}{HTML}{7678b0}

\newcommand{\floor}[1]{{\lfloor{#1}\rfloor}}
\newcommand{\abs}[1]{|#1|}
\newcommand{\norm}[1]{\Vert#1\Vert}
\newcommand{\bell}{\boldsymbol{\ell}}
\newcommand{\boldeta}{\boldsymbol{\eta}}
\newcommand{\bd}{\boldsymbol{d}}
\newcommand{\blambda}{\boldsymbol{\lambda}}
\newcommand{\balpha}{\boldsymbol{\alpha}}
\newcommand{\btheta}{\boldsymbol{\theta}}
\newcommand{\bnabla}{\boldsymbol{\nabla}}
\newcommand{\bLambda}{\boldsymbol{\Lambda}}
\newcommand{\bDelta}{\boldsymbol{\Delta}}
\newcommand{\bkappa}{\boldsymbol{\kappa}}
\newcommand{\bbeta}{\boldsymbol{\beta}}
\newcommand{\bdelta}{\boldsymbol{\delta}}
\newcommand{\bphi}{\boldsymbol{\phi}}
\newcommand{\bPhi}{\boldsymbol{\Phi}}
\newcommand{\bPi}{\boldsymbol{\Pi}}
\newcommand{\bpi}{\boldsymbol{\pi}}
\newcommand{\bChii}{\boldsymbol{\Chi}}
\newcommand{\bXi}{\boldsymbol{\Xi}}
\newcommand{\bxi}{\boldsymbol{\xi}}
\newcommand{\bGamma}{\boldsymbol{\Gamma}}
\newcommand{\bgamma}{\boldsymbol{\gamma}}
\newcommand{\bSigma}{\boldsymbol{\Sigma}}
\newcommand{\bsigma}{\boldsymbol{\sigma}}
\newcommand{\bPsi}{\boldsymbol{\Psi}}
\newcommand{\bpsi}{\boldsymbol{\psi}}
\newcommand{\bepsilon}{\boldsymbol{\epsilon}}
\newcommand{\bUpsilon}{\boldsymbol{\Upsilon}}
\newcommand{\bmu}{\boldsymbol{\mu}}
\newcommand{\bzeta}{\boldsymbol{\zeta}}
\newcommand{\bvarrho}{\boldsymbol{\varrho}}
\newcommand{\bvarphi}{\boldsymbol{\varphi}}
\newcommand{\bTheta}{\boldsymbol{\Theta}}
\newcommand{\bvartheta}{\boldsymbol{\vartheta}}
\newcommand{\bOmega}{\boldsymbol{\Omega}}
\newcommand{\bomega}{\boldsymbol{\omega}}
\newcommand{\prm}{^{\prime}}
\newcommand{\bB}{\boldsymbol{B}}
\newcommand{\bC}{\boldsymbol{C}}
\newcommand{\bc}{\boldsymbol{c}}
\newcommand{\bD}{\boldsymbol{D}}
\newcommand{\bff}{\boldsymbol{f}}
\newcommand{\bV}{\boldsymbol{V}}
\newcommand{\bG}{\boldsymbol{G}}
\newcommand{\bH}{\boldsymbol{H}}
\newcommand{\bmm}{\boldsymbol{m}}
\newcommand{\bM}{\boldsymbol{M}}
\newcommand{\bi}{\boldsymbol{i}}
\newcommand{\bI}{\boldsymbol{I}}
\newcommand{\bJ}{\boldsymbol{J}}
\newcommand{\bK}{\boldsymbol{K}}
\newcommand{\bk}{\boldsymbol{k}}
\newcommand{\bA}{\boldsymbol{A}}
\newcommand{\bS}{\boldsymbol{S}}
\newcommand{\bt}{\boldsymbol{t}}
\newcommand{\bT}{\boldsymbol{T}}
\newcommand{\bE}{\boldsymbol{E}}
\newcommand{\be}{\boldsymbol{e}}
\newcommand{\bp}{\boldsymbol{p}}
\newcommand{\bP}{\boldsymbol{P}}
\newcommand{\bq}{\boldsymbol{q}}
\newcommand{\bQ}{\boldsymbol{Q}}
\newcommand{\bR}{\boldsymbol{R}}
\newcommand{\bW}{\boldsymbol{W}}
\newcommand{\bu}{\boldsymbol{u}}
\newcommand{\bv}{\boldsymbol{v}}
\newcommand{\bs}{\boldsymbol{s}}
\newcommand{\bU}{\boldsymbol{U}}
\newcommand{\bx}{\boldsymbol{x}}
\newcommand{\bX}{\boldsymbol{X}}
\newcommand{\by}{\boldsymbol{y}}
\newcommand{\bY}{\boldsymbol{Y}}
\newcommand{\bZ}{\boldsymbol{Z}}
\newcommand{\bz}{\boldsymbol{z}}
\newcommand{\blda}{\boldsymbol{a}}
\newcommand{\bOO}{\boldsymbol{O}}
\newcommand{\bw}{\boldsymbol{w}}
\newcommand{\bee}{\boldsymbol{e}}
\newcommand{\bzero}{\boldsymbol{0}}
\newcommand{\lsb}{\bigl\{}
\newcommand{\rsb}{\bigr\}}
\newcommand{\bj}{{\bf{J}}}
\newcommand{\bone}{\boldsymbol{1}}
\newcommand{\bmV}{\boldsymbol{\mathcal V}}
\newcommand{\bmI}{\boldsymbol{\mathcal I}}
\newcommand{\bmJ}{\boldsymbol{\mathcal J}}
\newcommand{\mJ}{\mathcal J}
\newcommand{\mM}{\mathcal M}
\newcommand{\mR}{\mathcal R}
\newcommand{\mF}{\mathcal F}
\newcommand{\mC}{\mathcal C}
\newcommand{\one}{$\phantom{1}$}
\newcommand{\oo}{$\phantom{00}$}
\newcommand{\ooo}{$\phantom{000}$}
\newcommand{\oc}{$\phantom{0,}$}
\newcommand{\ooc}{$\phantom{00,}$}
\newcommand{\oooc}{$\phantom{000,}$}
\newcommand{\Ncand}{N_{\rm cand}}
\newcommand{\tover}{t_{\rm over}}
\newcommand{\tstd}{t_{\rm std,1}}
\newcommand{\ttwostage}{t_{\rm 2S,1}}
\newcommand{\psp}{P(S')}
\newcommand{\pep}{P(E')}
\newcommand{\pacc}{P_{\rm acc}}
\newcommand{\prob}{\mbox{I}\!\mbox{Pr}}
% \DeclareMathOperator*{\argmin}{argmin}
% \DeclareMathOperator*{\argmax}{argmax}
% \DeclareMathOperator*{\Cov}{Cov}
\newcommand{\argmax}{\operatornamewithlimits{argmax}}

\newcommand{\br}{\boldsymbol{r}}
\newcommand{\btau}{\boldsymbol{\tau}}
\newcommand{\bL}{\boldsymbol{L}}
\newcommand{\SNR}{\textnormal{SNR}}
\newcommand{\CNR}{\textnormal{CNR}}
\newcommand{\SE}{\textnormal{SE}}
\newcommand{\red}{\textcolor{red}}

\newcommand{\byR}{\boldsymbol{y}_R}
\newcommand{\byI}{\boldsymbol{y}_I}
\newcommand{\bvarepsilon}{\boldsymbol{\varepsilon}}
\newcommand{\beR}{\boldsymbol{\eta}_R}
\newcommand{\beI}{\boldsymbol{\eta}_I}
\newcommand{\bbh}{\boldsymbol{\hat{\beta}}}
\newcommand{\bah}{\boldsymbol{\hat{\alpha}}}
\newcommand{\bat}{\boldsymbol{\tilde{\alpha}}}
\newcommand{\btauh}{\boldsymbol{\hat{\tau}}}
\newcommand{\bbRh}{\boldsymbol{\hat{\beta}}_R}
\newcommand{\bbIh}{\boldsymbol{\hat{\beta}}_I}
\newcommand{\bbRt}{\boldsymbol{\tilde{\beta}}_R}
\newcommand{\bbIt}{\boldsymbol{\tilde{\beta}}_I}
\newcommand{\bxt}{\boldsymbol{x}_t}
\newcommand{\beRh}{\boldsymbol{\hat{\eta}}_R}
\newcommand{\beIh}{\boldsymbol{\hat{\eta}}_I}
\newcommand{\bbt}{\boldsymbol{\tilde{\beta}}}

\newcommand{\AIC}{\mbox{AIC}}
\newcommand{\BIC}{\mbox{BIC}}
\newcommand{\ICLBIC}{\mbox{ICL-BIC}}
\newcommand{\ben}{\begin{enumerate}}
\newcommand{\een}{\end{enumerate}}

% \newcolumntype{d}{@{}c@{\hspace{.03in}}}
\newcommand{\heightImage}{.73in}

%%% Additional Macro and command.
\newcommand{\E}{\mathbb{E}}
\newcommand{\pkg}[1]{{\fontseries{b}\selectfont #1}}
\makeatletter
\newcommand\code{\bgroup\@makeother\_\@makeother\~\@makeother\$\@codex}
\def\@codex#1{{\normalfont\ttfamily\hyphenchar\font=-1 #1}\egroup}
\makeatother
\let\proglang=\textsf
%%% End of additional Macro and command.

